CLIcK: A Benchmark Dataset of Cultural and Linguistic Intelligence in Korean

Despite the rapid development of large language models (LLMs) for the Korean language, there remains an obvious lack of benchmark datasets that test the requisite Korean cultural and linguistic knowledge. Because many existing Korean benchmark datasets are derived from the English counterparts through translation, they often overlook the different cultural contexts. For the few benchmark datasets that are sourced from Korean data capturing cultural knowledge, only narrow tasks such as bias and hate speech detection are offered. To address this gap, we introduce a benchmark of Cultural and Linguistic Intelligence in Korean (CLIcK), a dataset comprising 1,995 QA pairs. CLIcK sources its data from official Korean exams and textbooks, partitioning the questions into eleven categories under the two main categories of language and culture. For each instance in CLIcK, we provide fine-grained annotation of which cultural and linguistic knowledge is required to answer the question correctly. Using CLIcK, we test 13 language models to assess their performance. Our evaluation uncovers insights into their performances across the categories, as well as the diverse factors affecting their comprehension. CLIcK offers the first large-scale comprehensive Korean-centric analysis of LLMs' proficiency in Korean culture and language.

==> _1.Introduction/1.1introduction.tex <==
% Paragraph 1
As large language models (LLMs) are developed at an unprecedented pace, the imperative for establishing rigorous evaluation benchmarks becomes increasingly critical~\citep{}.
Yet, the current resources are confined to English-centric evaluation benchmarks, limiting to effectively assess the capabilities of LLMs in languages beyond English, including Korean.
Furthermore, the scarce Korean evaluation benchmarks that exist are primarily derived from translations of existing English standards, leading to the introduction of various artifacts. 
% For instance, the [...] dataset questions are originated from US/Western daily life, which is not a suitable source to evaluate a Korean LLM's performance even after translation~\citep{}. 
This discrepancy leads to consequently failing to offer an authentic assessment of performance in Korean-specific contexts~\citep{park2021klue,ma-etal-2022-encbp}.

% Paragraph 2
%As shown in Figure~\ref{}, [why simply translating an english dataset into Korean doesn't guarantee a well-formulated Korean evaluation benchmark]. 

\begin{figure}
    \centering
    \includegraphics[width=0.95\columnwidth]{rsc/intro.pdf}
    \caption{Overview of the CLIcK dataset creation and categorization process. Data is sourced from official exams and textbooks and validated by authors. The dataset is categorized into Korean Culture and Korean Language, further divided into various sub-categories. Sample questions highlight the superiority to mere translations, capturing nuances unique to the Korean context.}
    \label{fig:teaser_image}
\end{figure}

% Paragraph 3
To this end, we introduce \textbf{CLIcK}, a comprehensive evaluation benchmark encompassing 1,995 instances and 11 sub-categories, meticulously curated to probe deep into domains fundamental to Korean society such as law, economics, politics, and pop culture. Specifically, we divide into two different subsets, each associated with ``Korean Culture'' (8 sub-categories) and ``Korean Language'' (3 sub-categories).
Compared to previous Korean evaluation benchmarks, \textbf{CLIcK} broadens the spectrum of evaluation categories, necessitating a profound understanding of cultural nuances for precise linguistic evaluation~\citep{}.

% Paragraph 4
Using the \textbf{CLIcK} benchmark, we evaluate 12 different LLMs of diverse scales, including both multilingual LLMs and Korean-specific LLMs. Surprisingly, we find that LLaMA~\citep{touvron2023llama} mostly trained in English corpora outperforms Polyglot-Ko~\citep{ko2023technical}, that is specialized in Korean by a +2.82\% \& +4.47\% margin on the ``Korean Culture'' and ``Korean Language'' subset, respectively. Moreover, while proprietary LLMs outperform open-source LLMs across all 11 sub-categories, we also find that the gap is not significant on the History, Economy, and Function Language Usage sub-category, indicating the long-tailed characteristics of these sub-fields. Lastly, we highlight the robustness of our evaluation benchmark by (... flipping the order and changing prompts).

Our main contribution are summarized as follows:

%%%%%%%%%% Original Version %%%%%%%%%%
% The rise of Large Language Models (LLMs) highlights the need for comprehensive evaluation datasets.
% Existing datasets have become too simplistic for advanced LLMs, necessitating more complex and high-dimensional evaluation.e
% Furthermore, ~\citet{ma-etal-2022-encbp} shows the crucial influence of cultural information on an LLM's natural language understanding, emphasizing the importance of recognizing cultural backgrounds.
% Given these findings, the comprehension of cultural knowledge emerges as a critical evaluation factor for LLMs.
% % MMLU paper introduction 참고
% % category로 나뉜 것도 첫 문단에 넣기

% Several efforts have been made to evaluate language models specifically for the Korean language. However, a significant portion of the existing datasets have been translated from English versions~\cite{ham-etal-2020-kornli,jang-etal-2022-kobest}, potentially failing to capture Korea's unique nuances.
% There are few datasets that incorporate cultural aspects, and their limited public accessibility often presents a significant limitation. This scenario amplifies the demand for Korean-centric datasets that evaluate both linguistic and cultural aspects.% If the model was trained using the original English data, there's also a risk of overestimating its performance. This scenario amplifies the demand for datasets that evaluate Korean-centric aspects.\\

% In this work, we introduce and publicly release \textbf{CLIcK}\thinspace\footnote{\url{https://anonymous.4open.science/r/CLIcK/}}, a dataset tailored for fine-grained evaluation of Cultural and Linguistic Intelligence in Korean. %, using a multiple-choice QA format. 
% To achieve this, our data construction process is constructed in three primary stages. Initially, we derive the dataset from authentic Korean examinations and textbooks, ensuring CLIcK contains high-quality Korean-specific data. Then, the entire dataset is reviewed by four of the contributing authors, who are native Koreans. Finally, we categorize each instance in the dataset with a fine-grained label that captures which aspects of culture or the Korean language are required, enhancing CLIcK's fine-grained structure. 

% Using CLIcK, we evaluate 13 language models of diverse scales, including both multilingual and Korean-specialized models. Our evaluation reveals the intricate relationships between model type, scale, and the amount of Korean text used during training. Interestingly, many of these models find our dataset challenging. This emphasizes the unique value of CLIcK in providing a high-level evaluation of Korean linguistic and cultural contexts, facilitating in-depth analyses and comparisons of LLMs. 
%%%%%%%%%%

%analysis part
% The main contributions of this work are as follows:
\begin{itemize}
    \item We present CLIcK, a publicly available dataset designed to evaluate LLMs' cultural and linguistic understanding of Korean.
    \item We provide fine-grained categorization of the required knowledge to answer the queries in the dataset, enabling in-depth analyses and comparisons of LLMs.
    \item \textbf{\textit{{Analysis contribution, TBD}}}
\end{itemize}


==> rsc/Data_source2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[!ht]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lll|cccccccc|ccc|c@{}}
\toprule
\multicolumn{1}{l|}{\multirow{2}{*}{Source}}                                                                 & \multicolumn{1}{l|}{\multirow{2}{*}{Code}} & \multirow{2}{*}{TYPE}                               & \multicolumn{8}{l|}{Culture}                                                                                                                                                                                                          & \multicolumn{3}{l|}{Language}                                                             & \multicolumn{1}{l}{}    \\ \cmidrule(lr){4-14}
\multicolumn{1}{l|}{}                                                                                        & \multicolumn{1}{l|}{}                      &                                                     & \multicolumn{1}{l}{Tradition} & \multicolumn{1}{l}{Society} & \multicolumn{1}{l}{Law} & \multicolumn{1}{l}{Politics} & \multicolumn{1}{l}{Geo} & \multicolumn{1}{l}{History} & \multicolumn{1}{l}{Economy} & \multicolumn{1}{l|}{Pop} & \multicolumn{1}{l}{Concept} & \multicolumn{1}{l}{Grammar} & \multicolumn{1}{l|}{Function} & \multicolumn{1}{l}{SUM} \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Korean Immigration\\ and Integration Program\end{tabular}}    & \multicolumn{1}{l|}{KIIP}                  & \begin{tabular}[c]{@{}l@{}}Text\\ book\end{tabular} & O                             & O                           & O                       & O                            & O                       &                             & O                           & O                        &                             &                             &                               &                         \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}College Scholastic\\ Ability Test of Korea\end{tabular}}      & \multicolumn{1}{l|}{CSAT}                  & Exam                                                &                               &                             &                         &                              & O                       &                             &                             &                          & O                           & O                           & O                             &                         \\ \cmidrule(r){1-14}
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Test of Proficiency\\ in Korean\end{tabular}}                 & \multicolumn{1}{l|}{TOPIK}                 & Exam                                                &                               &                             &                         &                              &                         &                             &                             &                          & O                           & O                           &                               &                         \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}National Public Service\\ Examination - Grade 9\end{tabular}} & \multicolumn{1}{l|}{PSE}                   & Exam                                                &                               &                             &                         &                              &                         & O                           &                             &                          &                             &                             & O                             &                         \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Public Service \\ Aptitude Test\end{tabular}}                 & \multicolumn{1}{l|}{PSAT}                  & Exam                                                &                               &                             & O                       &                              &                         &                             &                             &                          &                             &                             &                               &                         \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Korean History Exam\\ Basic\end{tabular}}                     & \multicolumn{1}{l|}{KHB}                   & Exam                                                &                               &                             &                         &                              &                         & O                           &                             &                          &                             &                             &                               &                         \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Test of Teaching Korean\\ as a Foreign Language\end{tabular}} & \multicolumn{1}{l|}{Kedu}                  & Exam                                                & O                             & O                           & O                       &                              & O                       & O                           & O                           & O                        &                             & O                           &                               &                         \\ \midrule
                                                                                                             &                                            & Sum                                                 &                               &                             &                         &                              &                         &                             &                             &                          &                             &                             &                               &                         \\ \bottomrule
\end{tabular}
}
\caption{Sources for our data}
\label{tab:source2}
\end{table*}

==> rsc/Disc_Human.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[htb!]
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{@{}llllllll|l@{}}
\toprule
      &                                          & Polyglot & KULLM & KoAlpaca & Lamma & Gpt & Claude & Human \\ \midrule
PSE   & \multicolumn{1}{l|}{Language}     &          &       &          &       &     &        &       \\ \cmidrule(l){2-9} 
      & \multicolumn{1}{l|}{History}      &          &       &          &       &     &        &       \\ \midrule
PSAT  & \multicolumn{1}{l|}{Constitution} &          &       &          &       &     &        &       \\ \midrule
KHB   & \multicolumn{1}{l|}{History}      &          &       &          &       &     &        &       \\ \midrule
Kedu  & \multicolumn{1}{l|}{Language}     &          &       &          &       &     &        &       \\ \cmidrule(l){2-9} 
      & \multicolumn{1}{l|}{Culture}      &          &       &          &       &     &        &       \\ \bottomrule
\end{tabular}
}
\caption{Comparision with human level}
\label{Tab:disc_human}

\end{table*}

==> rsc/Disc_difficulty.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[htb!]
\centering
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
\multicolumn{4}{l}{Polyglot-Ko}                                                                                              \\ \midrule
1.3B          & 3.8B                               & 5.8B                                          & 12.8B                   \\ \midrule
1,449(75.1\%) & 1,362(68.3\%)                      & 1,307(65.5\%)                                 & 1,302(65.2\%)           \\ \hline\midrule
\multicolumn{2}{l|}{KULLM}                         & \multicolumn{2}{l}{KoAlpaca}                                            \\ \midrule
5.8B          & \multicolumn{1}{l|}{12.8B}         & 5.8B                                          & 12.8B                   \\ \midrule
1,225(61.4\%) & \multicolumn{1}{l|}{1,283(64.3\%)} & 1,259(63.1\%)                                 & 1,216(61.0\%)           \\ \hline\midrule 
\multicolumn{2}{l|}{LLaMA2-chat}                  & \multicolumn{1}{l|}{\multirow{2}{*}{GPT-3.5}} & \multirow{2}{*}{Claude} \\ \cmidrule(r){1-2}
5.8B          & \multicolumn{1}{l|}{12.8B}         & \multicolumn{1}{l|}{}                         &                         \\ \midrule
1,236(62.0\%) & \multicolumn{1}{l|}{1,226(61.4\%)} & \multicolumn{1}{l|}{739(37.0\%)}              &        695(34.8\%)                 \\ \bottomrule 
\end{tabular}
}
\caption{Proportion of challenging samples encountered by models of varying sizes.}
\label{tab:disc_diff}
\end{table}

==> rsc/Disc_entropy.tex <==
\begin{table*}[htb!]
\resizebox{\textwidth}{!}{%
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{tabular}{@{}cc|cccc|cc|cc|cc|c|c@{}}
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{}}                                                                        & \multicolumn{4}{c|}{Polyglot-Ko}                                                           & \multicolumn{2}{c|}{KULLM}                   & \multicolumn{2}{c|}{KoAlpaca}                & \multicolumn{2}{c|}{LLaMA}                   & \multirow{2}{*}{GPT-3.5} & \multirow{2}{*}{Claude} \\ \cmidrule(lr){3-12}
\multicolumn{2}{c|}{}                                                                                         & 1.3B                 & 3.8B                 & 5.8B                 & 12.8B                 & 5.8B                 & 12.8B                 & 5.8B                 & 12.8B                 & 7B                   & 13B                   &                          &                         \\ \midrule
\multicolumn{1}{c|}{}
\end{tabular}
}
\caption{Accuracy of the models per each category}
\label{Tab:acc_results}
\end{table*}
